A Robust Experimental Evaluation of Automated Multi-Label Classification Methods

Automated Machine Learning (AutoML) has emerged to deal with the selection and configuration of algorithms for a given learning task. With the progression of AutoML, several effective methods were introduced, especially for traditional classification and regression problems. Apart from the AutoML success, several issues remain open. One issue, in particular, is the lack of ability of AutoML methods to deal with different types of data. Based on this scenario, this paper approaches AutoML for multi-label classification (MLC) problems. In MLC, each example can be simultaneously associated to several class labels, unlike the standard classification task, where an example is associated to just one class label. In this work, we provide a general comparison of five automated multi-label classification methods -- two evolutionary methods, one Bayesian optimization method, one random search and one greedy search -- on 14 datasets and three designed search spaces. Overall, we observe that the most prominent method is the one based on a canonical grammar-based genetic programming (GGP) search method, namely Auto-MEKA$_{GGP}$. Auto-MEKA$_{GGP}$ presented the best average results in our comparison and was statistically better than all the other methods in different search spaces and evaluated measures, except when compared to the greedy search method.

==> src/backup_results.tex <==
\subsection{Experimental Results} \label{exp_results}

%This section perform an analysis of the results obtained by five \emph{search methods} described in Section \ref{sec:methods} in the 14 aforementioned datasets. Our analysis for these methods is based on three search spaces (i.e., Minimal, Medium and Large) and one execution time budget (i.e., five hours). Taking this information into account, 
Table \ref{measures-table} shows the average values, the average ranks  and the final statistical analysis for HL, RL and fitness measures, respectively. We indicate in bold the best average results. Besides, we take the the subscript names to  define the \emph{search methods}.

%Regarding the results of the EM measure, which is the most conservative, in Table \ref{em-table}, we observe for the \emph{search space} Minimal that the best average and rank value are found by Auto-MEKA$_{GGP}$, which is statistically superior than Auto-MEKA$_{RS}$ on this particular \emph{search space}. This statistical difference is indicated in Table~\ref{em-table} and in the following tables by the symbol $\succ$. For the \emph{search space} Medium, we have not found evidences of statistical differences, but whereas Auto-MEKA$_{BS}$ presented the best average value, Auto-MEKA$_{GGP}$ showed again the best average rank. In respect of the \emph{search space} Large, we identify that the best \emph{search methods} were Auto-MEKA$_{BO}$ and Auto-MEKA$_{GGP}$ based on the average value and rank, respectively. In addition, on this \emph{search space}, we have statistical evidences that Auto-MEKA$_{spGGP}$, Auto-MEKA$_{GGP}$ and Auto-MEKA$_{BO}$ are better methods than a pure random search (i.e., than Auto-MEKA$_{RS}$).

\begin{table}[!htbp]
\caption{Comparison of the hamming loss (to be minimized), ranking loss (to be minimized) and fitness (to be maximized) obtained by all \emph{search methods} in the test set for the three designed \emph{search spaces} with five hours of execution.}
\scriptsize
\begin{center}
\begin{tabular}{|l|l|l|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{\makecell[c]{Search \\ Space}}} & \multicolumn{1}{c|}{\textbf{\makecell[c]{Evaluated \\ Result}}} & \textbf{spGGP} & \textbf{GGP} & \textbf{BO} & \textbf{RS} & \textbf{BS} \\ \hline
\multicolumn{7}{|c|}{\textbf{Hamming Loss (HL)}} \\ \hline
\multicolumn{ 1}{|l|}{\textbf{Minimal}} & \textbf{Avg. Val.} & 0.135 & \textbf{0.134} & 0.208 & 0.137 & 0.135 \\ 
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 3.143 & \textbf{2.250} & 3.714 & 3.107 & 2.786 \\ 
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{no differences among all methods} \\ \cline{ 2- 7}
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{\textbf{Medium}} & \textbf{Avg. Val.} & 0.157 & 0.136 & \textbf{0.134} & 0.139 & 0.142 \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 4.036 & \textbf{2.251} & 2.607 & 3.00 & 3.107 \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{\{GGP\} $\succ$ \{spGGP\}, no differences among the others} \\ \cline{ 2- 7}
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{\textbf{Large}} & \textbf{Avg. Val.} & 0.137 & {0.134} & \textbf{0.130} & 0.143 & 0.139 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 3.214 & 2.571 & \textbf{2.07} & 4.00 & 3.142 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{\{BO\} $\succ$ \{RS\}, no differences among the others} \\ \hline
\multicolumn{7}{|c|}{\textbf{Ranking Loss (RL)}} \\ \hline
\multicolumn{ 1}{|l|}{\textbf{Minimal}} & Avg. Val. & \textbf{0.153} & 0.161 & 0.210 & 0.167 & 0.167 \\ 
 \multicolumn{ 1}{|l|}{} & Avg. Rank. & 2.321 & \textbf{2.214} & 3.750 & 3.429 & 3.286 \\ 
 \multicolumn{ 1}{|l|}{} & Stat. Comp. & \multicolumn{ 5}{c|}{no differences among all methods} \\ \cline{ 2- 7}
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{\textbf{Medium}} & Avg. Val. & \textbf{0.146} & 0.150 & 0.152 & 0.156 & 0.148 \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & Avg. Rank. & \textbf{2.679} & 2.821 & 3.250 & 3.321 & 2.929 \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & Stat. Comp. & \multicolumn{ 5}{c|}{no differences among all methods} \\ \cline{ 2- 7}
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{\textbf{Large}} & Avg. Val. & 0.147 & \textbf{0.135} & 0.149 & 0.157 & 0.140 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & Avg. Rank. & 2.821 & \textbf{2.536} & 2.786 & 4.071 & 2.786 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & Stat. Comp. & \multicolumn{ 5}{c|}{no differences among all methods} \\ \hline
\multicolumn{7}{|c|}{\textbf{Fitness}} \\ \hline
\multicolumn{ 1}{|l|}{\textbf{Min.}} & \textbf{Avg. Val.} & 0.626 & \textbf{0.631} & 0.590 & 0.624 & 0.626 \\ 
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 2.679 & \textbf{1.964} & 3.857 & 3.535 & 2.964 \\ 
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{\{GGP\} $\succ$ \{BO\}, no differences among the others} \\ \cline{ 2- 7}
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{\textbf{Med.}} & \textbf{Avg. Val.} & 0.634 & 0.639 & 0.626 & 0.629 & \textbf{0.645} \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 3.107 & \textbf{2.643} & 2.929 & 3.429 & 2.893 \\ 
\rowcolor{gray!20}
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{no differences for all methods} \\ \cline{ 2- 7}
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{\textbf{Larg.}} & \textbf{Avg. Val.} & 0.632 & \textbf{0.635} & \textbf{0.635} & 0.626 & 0.632 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & \textbf{Avg. Rank.} & 2.607 & \textbf{2.429} & 2.571 & 4.286 & 3.107 \\ 
\rowcolor{gray!50}
 \multicolumn{ 1}{|l|}{} & \textbf{Stat. Comp.} & \multicolumn{ 5}{c|}{\{spGGP, GGP, BO\} $\succ$ \{RS\}, no differences among the others} \\ \hline
\end{tabular}
\end{center}
\label{measures-table}
\end{table}

%These results for the EM measure indicate indeed what we expected, i.e., the size of the \emph{search space} affects the performance of the \emph{search methods}.  In other words, by giving an enough time budget to the \emph{search methods}, only robust search methods could deal better with the tradeoff between exploration and exploitation, beating the random search method (i.e., Auto-MEKA$_{RS}$) in large \emph{search spaces}. Furthermore, we observe that Auto-MEKA$_{GGP}$) was the only method to beat  Auto-MEKA$_{RS}$ in two search spaces, showing its search capabilities.

The results for the HL measure with five hours, in Table \ref{measures-table}, showed that Auto-MEKA$_{GGP}$ had the best average values and ranks in the \emph{search space} Minimal, but it had only the best average rank in the \emph{search space} Medium.  Complementary, Auto-MEKA$_{BO}$ showed the best average value  and Auto-MEKA$_{GGP}$ indicated to be statistically better than Auto-MEKA$_{spGGP}$ in the \emph{search space} Medium. Nonetheless, there is no indication of statistical difference for the other cases of \emph{search space} Medium, neither for all cases of Minimal. When considering the \emph{search space} Large, Auto-MEKA$_{BO}$ had the best average value and the best average rank. In fact, Auto-MEKA$_{BO}$ was the only \emph{search method} to present statistical better results when compared to Auto-MEKA$_{RS}$ in this \emph{search space}.  

For the HL measure, we also note that the size of the \emph{search space} has a strict influence on the performance of the \emph{search method}. By looking at the statistical results of Table \ref{measures-table}, we can conclude that only Auto-MEKA$_{BO}$ was able to beat Auto-MEKA$_{RS}$ for the \emph{search space} Large. In the other cases, we do not see an indication of the \emph{search methods} to tradeoff well between exploration and exploitation.

%Furthermore, we evaluated the results of the \emph{search methods} in the \emph{search spaces} on a measure that is commonly used in the single-label scenario, and adapted for the multi-label context, i.e., the FM measure. Table \ref{measures-table} also shows the results for FM, indicating that the best average rank and value in the \emph{search space} Minimal was achieved by  $\text{Auto-MEKA}_{GGP}$. In the case of the \emph{search space} Medium, $\text{Auto-MEKA}_{BS}$ presented the best average value and also the best average rank. Similarly to the \emph{search space} Minimal,
%the best average value and rank were found by $\text{Auto-MEKA}_{GGP}$ in the \emph{search space} Large.
%Nevertheless, in this particular measure, no method was statistically better than other in the designed \emph{search spaces}. We claim that this flat result was caused by the nature of the FM measure, which was not specifically designed to evaluate MLC classifiers, but SLC classifiers instead.

In addition, Table \ref{measures-table} summarizes the results for the evaluation measure from a different evaluation context, i.e., RL. Whilst $\text{Auto-MEKA}_{spGGP}$ was the  \emph{search method} with the best average value in the \emph{search space} Minimal, $\text{Auto-MEKA}_{GGP}$ achieved the best average rank in this scenario. Distinctly, $\text{Auto-MEKA}_{spGGP}$ selected and configured MLC algorithms in such way they produced the best average value and rank in the \emph{search space} Medium. For the \emph{search space} Large, $\text{Auto-MEKA}_{GGP}$ turned into the \emph{search methods} with the best average value and the best average rank.

The results of RL did not present any evidence of statistical significance. Therefore, the \emph{search methods } did not differ from each other. As this metric comes from another context, we would like to understand why it presented such a flat result for all \emph{search spaces} and \emph{search methods}. Our claim stands for the RL measure being way conservative and not showing sensibility of different multi-label classifiers. As it only penalizes reversed pair of labels into the ranking and  does not take into account the label-pair depth into the ranking to penalize, this can make this measure not good enough to be used in isolation to evaluate MLC algorithms. In future work, it might be interesting to evaluate whether this measure is appropriate to be part of our study or whether we should consider a rank-based measure that takes into account the depth of the ranking (e.g., coverage).

HL and RL are measures that compose the fitness/quality function. We also analyse the results of the fitness measure to have a better assessment of the results of \emph{search methods}. With respect to the \emph{search space} Minimal, Auto-MEKA$_{GGP}$ presented the best average value and also the best average rank. Besides, we found statistical evidences that Auto-MEKA$_{GGP}$ has better results than Auto-MEKA$_{BO}$ in this \emph{search space}. In the \emph{search space} Medium, we observe that Auto-MEKA$_{GGP}$ produced the best average ranking and Auto-MEKA$_{BS}$ presented the best average value. Finally, the results regarding the \emph{search space} Large for the fitness measure are similar to those found for the EM measure. In this case, Auto-MEKA$_{spGGP}$, Auto-MEKA$_{GGP}$ and  Auto-MEKA$_{BO}$ achieved better results than  Auto-MEKA$_{RS}$, showing their capabilities to handle enormous \emph{search spaces} -- when giving enough time for them to proceed with their searches. Apart from the statistical results, we can observe in Table \ref{fitness-table} that Auto-MEKA$_{GGP}$ also reached the best average value and rank with one and five hours. Furthermore, Auto-MEKA$_{BO}$ had even results to Auto-MEKA$_{GGP}$ in terms of the average value. 

We can now provide overall conclusions based on the results of this section. Ee believe that the size of the \emph{search spaces} explored/exploited by the \emph{search methods} influenced in the multi-label classification. We understand that for smaller \emph{search spaces} (e.g., Minimal and Medium), the  \emph{search methods} have more facilities to proceed with their searches and, as a result of that, their results become broadly similar among each other. When we increase the \emph{search space} to Large, only those with robust search mechanisms could deal better with the tradeoff between exploration and exploration, making them to achieve competitive results.

%the \emph{search methods} that robust enough could beat Auto-MEKA$_{RS}$.

However, we believe the robust methods (i.e., those based on the evolutionary and Bayesian optimization frameworks) can still improve their final predictive performances as they could not beat the beam \emph{search method}, a pure-exploitation method. This also happened against the random \emph{search method} in some cases. Thus, these \emph{search methods} still could not satisfactorily balance between exploration and exploitation. In our perspective, this would occur if they could beat simultaneously Auto-MEKA$_{RS}$ and Auto-MEKA$_{BS}$. For the \emph{search spaces} Minimal and Medium, this result is more understandable. The smaller the \emph{search space}, the easier is to perform the search on them. This end to in better results for Auto-MEKA$_{RS}$ and Auto-MEKA$_{BS}$ in such a way the other \emph{search methods} could not be statistically different from both of them. For bigger \emph{search spaces} (e.g., Large), this should be the opposite. As they present robust search mechanisms, they should guarantee statistically better results against pure-exploration and pure-exploitation \emph{search methods}. 



